First Hitting Diffusion Models for Generating Manifold, Graph and Categorical Data

We propose a family of First Hitting Diffusion Models (FHDM), deep generative models that generate data with a diffusion process that terminates at a random first hitting time. This yields an extension of the standard fixed-time diffusion models that terminate at a pre-specified deterministic time. Although standard diffusion models are designed for continuous unconstrained data, FHDM is naturally designed to learn distributions on continuous as well as a range of discrete and structure domains. Moreover, FHDM enables instance-dependent terminate time and accelerates the diffusion process to sample higher quality data with fewer diffusion steps. Technically, we train FHDM by maximum likelihood estimation on diffusion trajectories augmented from observed data with conditional first hitting processes (i.e., bridge) derived based on Doob's $h$-transform, deviating from the commonly used time-reversal mechanism. We apply FHDM to generate data in various domains such as point cloud (general continuous distribution), climate and geographical events on earth (continuous distribution on the sphere), unweighted graphs (distribution of binary matrices), and segmentation maps of 2D images (high-dimensional categorical distribution). We observe considerable improvement compared with the state-of-the-art approaches in both quality and speed.

==> pratenddefaultcategory.tex <==

\label{proofsection:prAtEndii}\begin{proof}[Proof of \autoref{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}As $\Q ^{B_d}$ is a product of identical and independent one-dimensional processes, it is sufficient to consider the one dimension case $d=1$, in which case the process is a Brownian motion $ \d Z_t =\d W_t$ starting from interval $Z_0 \in [0,1]$ and stopped $\tau =\min _{t} \{t\colon ~Z_t \not \in (0,1)\}$ when it exits the interval. Hence, the Poisson kernel is $$ \dist Q^\binary _\Omega ( x ~|~ z) = \prob (W_\tau =x ~|~ W_{t} = z) = \prob (W_\tau =x ~|~ W_{t} = z),~~~~\forall x\in \{0,1\} $$ Then, it is a textbook result that $\prob (W_\tau =x ~|~ W_{t} = z) = x z + (1-x) (1-z) = \ber (x|z).$ See e.g., Eq.~3.0.4, Page 212 of \citet {borodin2015handbook}.\end{proof}
\label{proofsection:prAtEndiii}\begin{proof}[Proof of \autoref{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}It is a straightforward application of formula \eqref {equ:Xtr} in the case of $b_t = 0$, $\sigma _t(Z_t) = \ind (\norm {Z_t} <1)$ and $q_\Omega (x|z) = \frac {1-\norm {z}^2}{\norm {x-z}^d}$ as shown in \eqref {equ:PoissonSd}.\end{proof}
\label{proofsection:prAtEndiv}\begin{proof}[Proof of \autoref{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}It is a straightforward application of formula \eqref {equ:Xtr} in the case of $b_t = 0$, $\sigma _t(Z_t) = \mathrm {diag}(\ind (Z_t\in (0,1)))$ and $\Q _\Omega (x|z) =\ber (x|z)$ as shown in Proposition~\eqref {thm:ber}.\end{proof}
\label{proofsection:prAtEndv}\begin{proof}[Proof of \autoref{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}This is the standard result on Brownian bridge. In particular, we just need to note that $(Z_{T} ~|~Z_t=z) \sim \normal (z, ~T-t)$ and apply formula \eqref {equ:Xtr}.\end{proof}
\label{proofsection:prAtEndvi}\begin{proof}[Proof of \autoref{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}Eq.~\eqref {equ:schr} is the direct result of $\Q ^\tg = \argmin _{\P } \KL (\P ~||~ \Q ^\tg )$, and that $$\KL (\P ~||~ \Q ^\tg ) \equiv \KL (\P ~||~\Q ) - \E _{\P }[\log \tgd (\X _\tau )], $$ where we used $\Q ^\tg (\d Z) = \Q (\d Z) \pi ^*(Z_\tau )$. \par Eq~\eqref {equ:sch} is a simple consequence of the disintegration theorem. Note that any $\P $ that satisfies $\P _\Omega = \tg $ can be written into $\P (\d \X ) = \tg (\d \X _\tau ) \P (\d \X ~|~ \X _\tau )$. By the chain rule of KL divergence, \bbb \label {equ:chainKL} \KL (\P ~||~\Q ) = \KL (\tg ~||~\Q _\Omega ) + \E _{\X _\tau \sim \tg }\left [ \KL (\P ( \cdot | \X _\tau ) ~||~ \Q (\cdot |\X _\tau )) \right ]. \eee Since it is constrained that $\P _\Omega = \tg $, the optimal $\P $ is determined by the choice of $\P (\cdot | Z_\tau )$ and it should yield $\P (\d \X ~|~ \X _\tau ) = \Q (\d \X ~|~ \X _\tau )$. Therefore, the optimal $\P $ is $\tg (Z_\tau ) \Q (\cdot |Z_{\tau }) = \Q ^\tg $. \par In fact, by the same derivation, we can see that \eqref {equ:sch} remains correct if we replace $\KL (\P ~||~\Q )$ with $\KL (\Q ~||~\P )$.\end{proof}
\label{proofsection:prAtEndvii}\begin{proof}[Proof of \autoref{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Denote by $\Q ^x = \Q (\cdot | Z_\tau = x)$. Let $p^\theta $ be the density function of $\P ^\theta $ w.r.t. to some reference measure (e.g., $\Q ^\tg $). We have \bb \KL (\Q ^\tg ~||~ \P ^\theta ) & = -\E _{Z \sim \Q ^\tg } [\log p^{\theta }(Z)] + \const \\ & = - \E _{x\sim \tg } \E _{Z\sim \Q ^x} [\log p^{\theta }(Z)] + \const \\ & = \E _{x\sim \Pi ^*}\left [ \KL (\Q ^x ~||~ \P ^\theta ) \right ] +\const , \ee where $ \KL (\Q ^x ~||~ \P ^\theta )$ can be evaluated using Girsanov theorem, \bb \KL (\Q ^x ~||~ \P ^\theta ) & = \KL (\Q ^x_0 ~||~ \P ^\theta _0) + \frac {1}{2} \E _{Z\sim \Q ^x} \left [\int _0^\tau \norm {s^\theta _t(Z_t) - b_t(Z_t|x)}^2_2 \dt \right ] \\ & = \E _{Z\sim \Q ^x}\left [ -\log p_0^\theta (Z_0) + \frac {1}{2} \int _0^\tau \norm {s^\theta _t(Z_t) - b_t(Z_t|x)}^2_2 \dt \right ] + \const . \ee Hence \bb \L (\theta ) & = \E _{x\sim \tg , Z\sim \Q ^x}\left [ -\log p_0^\theta (Z_0) + \frac {1}{2} \int _0^\tau \norm {s^\theta _t(Z_t) - b_t(Z_t|x)}^2_2 \dt \right ] + \const \\ & = \E _{Z\sim \Qt }\left [ -\log p_0^\theta (Z_0) + \frac {1}{2} \int _0^\tau \norm {s^\theta _t(Z_t) - b_t(Z_t|Z_\tau )}^2_2 \dt \right ] + \const . \ee \end{proof}
\label{proofsection:prAtEndviii}\begin{proof}[Proof of \autoref{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}Assume $\norm {f}_\infty \defeq \sup _{t\in [0+\infty ), x\in [0,1]^d}\norm {f_t(x)}_2 < +\infty $. Consider the following two processes with the same initialization: \bbb \label {equ:q0} \begin {split} & \Q ^0 \colon \d Z_t = \ind (Z_t\in (0,1)) \circ \left ( \dd _{z}\log \mathrm {Ber}(\Omega ~|~Z_t) \dt + \d W_t \right ) \\ & \Q ^f \colon \d Z_t = \ind (Z_t\in (0,1)) \circ \left ( f_t^\theta (Z_t) ~+~ \dd _{z}\log \mathrm {Ber}(\Omega ~|~Z_t) \dt + \d W_t \right ). \end {split} \eee Girsanov theorem shows that $\KL (\Q ^0~||~ \Q ^f) = \frac {1}{2}\E _{\Q ^0}[\int _0^\tau \norm {f_t (Z_t)}^2] \leq \frac {1}{2}\norm {f}^2_\infty \E _{\Q ^0}[\tau ] <+\infty $, where we used the fact that the expected hitting time $\E _{\Q ^0}[\tau ]$ of $\Q ^0$ is finite (see Lemma~\ref {lem:hehq0} below). \par Now $\KL (\Q ^0~||~ \Q ^f)<+\infty $ implies that that $\Q ^0$ and $\Q ^f$ has the same support. Hence the fact that $\Q ^0$ guarantees to hit $\Omega $ when exiting $V$, i.e., $\Q ^0(Z_\tau \in \Omega ) =1$, when exit implies that $\Q ^f$ has the same property, i.e., $\Q ^f(Z_\tau \in \Omega ) =1$. \begin {lem}\label {lem:hehq0} Let $\tau ^0 = \inf \{ t\colon Z_t \in \Omega \}$ be the first hitting time to $\Omega \subseteq \{0,1\}^d$ of the the process $\Q ^0$ in Eq.~\eqref {equ:q0}. Then $\E [\tau ^0]<+\infty $. \end {lem} \begin {proof} Consider the following two processes starting from the same deterministic initialization $Z_0 = Y_0 = z_0\in (0,1)^d$: \bb & \Q ^0 \colon \d Z_t = \ind (Z_t\in (0,1)) \circ \left ( \dd _{z}\log \mathrm {Ber}(\Omega ~|~Z_t) \dt + \d W_t \right ) \\ & \Q ^* \colon \d Y_t = \ind (Y_t\in (0,1)) \circ \left ( \d W_t \right ). \ee Denote by $\tau ^0$ and $\tau ^*$ the corresponding hitting times to $\Omega $, that is, $\tau ^0 = \inf \{t \colon Z_t \in \Omega \}$, and $\tau ^* = \inf \{t \colon Y_t \in \Omega \}$. \par Then we know from $h$-transform that $\Q ^0$ is the conditioned process of $\Q ^*$ given that $Z_\tau \in \Omega $, that is, $ \Q ^0 = \Q ^*(\cdot ~|~ Z_\tau \in \Omega )$. \par \par \par Therefore, the first hitting time $\tau ^0$ of $\Q ^0$ has the same law as that of $\tau ^* ~|~ Y_\tau \in \Omega $, that is, $\Q ^0 (\tau ^0 \in A) = \Q ^*(\tau ^* \in A ~|~ Y_\tau \in \Omega )$ for any measurable set $A\subseteq [0, +\infty )$. \par But we know that $\E [\tau ^*~|~ Y_\tau \in \Omega ] <+\infty $ due to the diffusion nature of Brownian motion. Hence, $\E [\tau ^0] = \E [\tau ^*~|~ Y_\tau \in \Omega ] < +\infty $. \end {proof}\end{proof}

